Navigating Spatio-Temporal Heterogeneity: A Graph Transformer Approach for Traffic Forecasting

Traffic forecasting has emerged as a crucial research area in the development of smart cities. Although various neural networks with intricate architectures have been developed to address this problem, they still face two key challenges: i) Recent advancements in network designs for modeling spatio-temporal correlations are starting to see diminishing returns in performance enhancements. ii) Additionally, most models do not account for the spatio-temporal heterogeneity inherent in traffic data, i.e., traffic distribution varies significantly across different regions and traffic flow patterns fluctuate across various time slots. To tackle these challenges, we introduce the Spatio-Temporal Graph Transformer (STGormer), which effectively integrates attribute and structure information inherent in traffic data for learning spatio-temporal correlations, and a mixture-of-experts module for capturing heterogeneity along spaital and temporal axes. Specifically, we design two straightforward yet effective spatial encoding methods based on the graph structure and integrate time position encoding into the vanilla transformer to capture spatio-temporal traffic patterns. Additionally, a mixture-of-experts enhanced feedforward neural network (FNN) module adaptively assigns suitable expert layers to distinct patterns via a spatio-temporal gating network, further improving overall prediction accuracy. Experiments on real-world traffic datasets demonstrate that STGormer achieves state-of-the-art performance.

==> sections/gohst.tex <==
Traffic forecasting has emerged as a crucial research area in the development of smart cities. Although various neural networks with intricate architectures have been developed to address this problem, they still face two key challenges: i) Recent advancements in network designs for modeling spatio-temporal correlations are starting to see diminishing returns in performance enhancements. ii) Additionally, most models do not account for the spatio-temporal heterogeneity inherent in traffic data, i.e., traffic distribution varies significantly across different regions and traffic flow patterns fluctuate across various time slots. To tackle these challenges, we introduce the Spatio-Temporal Graph Transformer (STGormer), which effectively integrates attribute and structure information inherent in traffic data for learning spatio-temporal correlations, and a mixture-of-experts module for capturing heterogeneity along spaital and temporal axes. Specifically, we design two straightforward yet effective spatial encoding methods based on the graph structure and integrate time position encoding into the vanilla transformer to capture spatio-temporal traffic patterns. Additionally, a mixture-of-experts enhanced feedforward neural network (FNN) module adaptively assigns suitable expert layers to distinct patterns via a spatio-temporal gating network, further improving overall prediction accuracy. Experiments on five real-world datasets demonstrate that STGormer achieves state-of-the-art performance. 



\section{Introduction}
% 交通预测的重要性
Recent advancements in perception technologies and computational environments have spurred the emergence of diverse big data types in urban settings, encompassing traffic flow, meteorological conditions, individual movement patterns, and social media interactions. 
Among these, traffic forecasting has emerged as a particularly significant area, attracting extensive interest from both academia and industry due to its crucial implications for urban traffic management and planning.

% 交通流量在temporal和spatial维度的特点
This research area is marked by the need to decipher complex temporal and spatial patterns~\cite{guo2021hierarchical}, with the temporal aspect often exhibiting cyclical trends on a daily or weekly basis, and the spatial dimension characterized by the connectivity and interactions among various urban locations~\cite{shao2022pre}.
Figure~\ref{fig:1-motivation-s} shows the traffic flow from sensors 20, 110, and 301 in the PEMS04 dataset over the same time frame. Sensors 20 and 301 exhibit very similar patterns due to their proximity within the traffic network, while sensor 110 displays distinct trends, indicating spatial heterogeneity. 
Figure~\ref{fig:1-motivation-t} provides a detailed view of the traffic flow data from sensor 20 over one week, revealing distinct weekday and weekend traffic patterns particularly during peak hours. Weekdays show a pronounced morning rush hour peak, while weekends exhibit a more uniform distribution throughout the day without significant peaks, highlighting the temporal heterogeneity in weekly patterns.

% 先前的研究工作
% STGNN 优缺点
To overcome the challenges related to spatio-temporal modeling, Spatial-Temporal Graph Neural Networks (STGNNs) have garnered significant attention for their accuracy in predictions~\cite{bai2019stg2seq}. 
They integrate Graph Neural Networks (GNNs)~\cite{kipf2016semi} with sequential models~\cite{sutskever2014sequence,yu2019review}, where the former captures dependencies among time series, the latter identifies temporal patterns. 
By effectively modeling both spatial and temporal characteristics, STGNNs have consistently delivered state-of-the-art results. 
While STGNN models recognize that flow patterns are closely tied to spatial relations and specific time intervals, they often struggle to clearly distinguish spatial and temporal heterogeneity.
% Attention模型的优缺点
Other studies have incorporated attention models to enhance dynamic spatial modeling, taking advantage of no spatial constraints, as exemplified by GMAN~\cite{zheng2020gman} and STAEformer~\cite{liu2023spatio}. Although attention-based models fuse the spatio-temporal representation with one step, recent research has shown that they frequently struggle to generate meaningful attention maps, instead diffusing attention weights across all nodes~\cite{jin2022visual}. Moreover, these models often overlook spatial structural information embedded within graphs during attention computation.

